Improving Long Handwritten Text Line Recognition with Convolutional Multi-way Associative Memory

Convolutional Recurrent Neural Networks (CRNNs) excel at scene text recognition. Unfortunately, they are likely to suffer from vanishing/exploding gradient problems when processing long text images, which are commonly found in scanned documents. This poses a major challenge to goal of completely solving Optical Character Recognition (OCR) problem. Inspired by recently proposed memory-augmented neural networks (MANNs) for long-term sequential modeling, we present a new architecture dubbed Convolutional Multi-way Associative Memory (CMAM) to tackle the limitation of current CRNNs. By leveraging recent memory accessing mechanisms in MANNs, our architecture demonstrates superior performance against other CRNN counterparts in three real-world long text OCR datasets.

==> intro_v1.tex <==
Handwritten Optical Character Recognition (HOCR) is a challenge task as it requires both visual processing and sequential learning to transcript an image of handwritten text. Compared to printed OCR, HOCR is harder because one character can be written in many forms depending on the style of the writer. 

Recent success of deep learning and particularly, Convolutional Neural Networks (CNNs) in computer vision \cite{krizhevsky2012imagenet,simonyan2014very} has motivated the use of CNNs in solving the visual processing part of OCR problems. Many recent researches have confirmed the advantage of using CNNs \cite{jaderberg2016reading,wang2017gated}, making it a standard visual feature extractor for various OCR problems including HOCR.  

The remaining problem in HOCR is to capture the sequential relationships amongst visual features, which is highly important to achieve good recognition performance, especially when the visual features are not enough to determine the recognition output (e.g, in noisy or context-dependent settings). To cope with this problem, many attempts have been made including using Hidden Markov Models (HMM) \cite{suryani2016benefits} or equipping Recurrent Neural Networks (RNN) with Connectionist Temporal Classification (CTC) \cite{graves2009offline}. Recently, Bidirectional Long Short-term Memory (BiLSTM) \cite{hochreiter1997long, schuster1997bidirectional}  has emerged as a powerful sequential model for OCR, achieving state-of-the-arts in a wide range of OCR tasks \cite{chowdhury2018efficient,puigcerver2017multidimensional,shi2017end}. 

Despite the promising empirical results, BiLSTM as well as other RNN-based models is  incapable of remembering long context due to vanishing/exploding gradient problems \cite{bengio1994learning,pascanu2013difficulty}. Current HOCR datasets, which contains only scene text or short segments of texts are not challenging enough to expose BiLSTM's weekness. However, when approaching industrial problems, which often involve transcription of the whole line of documents written in complicated languages, RNN-based models may fail to achieve good results. In this paper, we present a novel model named Convolutional Associative Memory (CAM) that tackles the limitation of RNN-based methods in HOCR. 

More specifically, we adapt recent memory-augmented neural networks (MANNs) by integrating an external memory module into convolution and CTC layers. The CNN layers read the input image, encoding it to a sequence of visual features. At each timestep of the sequence, a BiLSTM controller will be used to store the feature into the memory, access the memory and generate an output. The output will be passed to CTC layer to produce the CTC loss and the final predicted character.  Moreover, to make the architecture fit with HOCR tasks, we introduce efficient memory accessing mechanisms built upon Diffrentiable Neural Computer (DNC) \cite{graves2016hybrid}, a strong and fully differentiable MANN. Through extensive experiments on both public English and industrial Japanese handwritten datasets, we demonstrate empirical evidences showing that our architecture provides better accuracy, when compared to the current state-of-the-art BiLSTM.   

==> related_v1.tex <==

\subsection{Segmentation-based Methods }

Traditional approaches attempt to break the problem into three phases:
character segmentation, character recognition and segmentation-recognition
integration. For segmentation problem, solutions involve histogram
projecting {[}9{]}, connected component {[}3, 7{]}, hand-craft feature
designs for specific languages {[}2, 11{]} and lexicon-driven segmentation
{[}1{]}. These methods try to split the whole line images into consecutive
primitive segments, each of which will be recognized by another classifier.
Some works make use of modified quadratic discriminant function (MQDF)
{[}5{]} and nearest prototype classifier (NPC) {[}6{]} for classification
step. Recently, deep neural network such as Convolution Neural Network
(CNN) is adapted to Japanese OCR problem and shows promising results
in {[}4, 8{]}. The integration problem can be formulated as finding
the optimal candidate segmentation-recognition path, where each candidate
is usually evaluated by combining the character recognition scores
(classifier outputs), geometric context, and linguistic context {[}7{]}.
Although these methods work well in some applications, the solutions
are not end-to-end and often require human feature engineering. Also,
separation of segmentation and recognition makes the performance depends
heavily on segmentation step. This is risky since character segmentation
for complex languages such as Japanese and Chinese is challenging
{[}10{]}. Lastly, these approaches are not time-efficient since segmentation
and optimal path searching phases are time-consuming in inference
{[}7{]}. 

\subsection{Segmentation-free Methods }

Opposing to traditional segmentation-based methods, these new approaches
train the model end-to-end without segmentation step. Most of them
use CNN layers for image feature extractions, including lexicon-driven
{[}20{]} or lexicon-free {[}21{]} methods. Other works apply temporal
models to jointly learn the sequence of image features. One example
involves combining CNN wih Hidden Markov Model in {[}14{]}. Long-Short
Term Memory (LSTM) with Connectionist Temporal Classification (CTC)
{[}12{]} is naturally combined with CNN in {[}13{]}, which achieves
state-of-the-art in recognizing English characters image in wild-scene.
Authors in {[}17{]} proposes using CNN with sliding window and replacing
Dropout with Maxout Layer, achieving good results for handwriting
Japanese characters. Another alternative approach is to apply directly
2D LSTM for feature extraction and sequential learning at once. This
approach gains promising results in handwriting Arab {[}15{]} and
Chinese {[}16{]} language. Recently, there are some attempts that
replacing CTC with Seq2Seq architecture, both without {[}18{]} and
with attention mechanism {[}19{]}. The initial results give competitive
performance relative to CTC output while being executed in more natural
settings. Hybrid model between CTC and attention decoder {[}23{]}
is also proposed and gain big improvement in Chinese and Japanese
speech recognition. Latest researches explore new architecture of
CNN for better OCR feature extraction such as Recursive CNN with attention
{[}22{]} or Gated Recurrent CNN {[}24{]} for English OCR in the wild.

\subsection{Memory-augmented Neural Networks}
Memory augmented neural networks (MANN) have emerged as a new promising
research topic in deep learning. MANNs are proven to be better than their LSTM counterparts with both empirical evidences \cite{graves2014neural,graves2016hybrid,10.1007/978-3-319-93040-4_22} and theoretical motivations \cite{gulcehre2017memory, le2018learning}. For practical applications, MANNs have been applied to many problems such as meta learning \cite{santoro2016meta}, question answering \cite{miller2016key}, healthcare \cite{10.1007/978-3-319-93040-4_22,Le:2018:DMN:3219819.3219981} and dialog system \cite{le2018variational}. However, for OCR-related problems, there is limited work applying MANN. Our work is one of the first attempts that utilize MANN for HOCR tasks. 

